OGMP: Oracle Guided Multi-mode Policies for Agile and Versatile Robot Control

The efficacy of reinforcement learning for robot control relies on the tailored integration of task-specific priors and heuristics for effective exploration, which challenges their straightforward application to complex tasks and necessitates a unified approach. In this work, we define a general class for priors called oracles that generate state references when queried in a closed-loop manner during training. By bounding the permissible state around the oracle's ansatz, we propose a task-agnostic oracle-guided policy optimization. To enhance modularity, we introduce task-vital modes, showing that a policy mastering a compact set of modes and transitions can handle infinite-horizon tasks. For instance, to perform parkour on an infinitely long track, the policy must learn to jump, leap, pace, and transition between these modes effectively. We validate this approach in challenging bipedal control tasks: parkour and diving using a 16 DoF dynamic bipedal robot, HECTOR. Our method results in a single policy per task, solving parkour across diverse tracks and omnidirectional diving from varied heights up to 2m in simulation, showcasing versatile agility. We demonstrate successful sim-to-real transfer of parkour, including leaping over gaps up to 105 % of the leg length, jumping over blocks up to 20 % of the robot's nominal height, and pacing at speeds of up to 0.6 m/s, along with effective transitions between these modes in the real robot.

==> sections/related_works.tex <==
\section{Related works}
\label{sec:related_works}

\textbf{Guided Policy Optimisation (GPO)}: aims to improve the sample efficiency and mitigate poor local optima in direct policy optimization, broadly classified into Control-guided and Reference-guided methods. \emph{Control-guided} methods use control trajectories to guide the optimization. \cite{levine2013guided} generates guiding samples with prior controllers, while \cite{levine2014lerning} enforces policy-trajectory constraints to discover complex behaviors. \cite{mordatch2014combining} alternates between trajectory optimization and regression in deterministic settings, and \cite{cheng19control} minimizes RL policy variance with a regularized control law. Using model-based controllers \cite{carius2020mpcnet} proposed a control Hamiltonian minimizing imitation learning, and \cite{gangapurwala2020guided} studied constrained GPO with varying intensity constraints validated in quadrupedal walking. Recently, \cite{jenelten2023dtc} demonstrated precise and robust quadrupedal locomotion with a low-level tracking policy guided by non-linear MPC. However, these methods require pre-existing control, limiting their applicability to tasks (like parkour) without an a priori feasible controller. \emph{Reference-guided} methods use state-reference trajectories to guide RL and emergently learn the optimal actions. \cite{peng2018deep} proposed an example-guided approach for physics-based character control from morphologically similar demonstrations and was applied to real-robot bipedal locomotion in \cite{li2024reinforcement}. \cite{peng2021amp} further extended \cite{peng2018deep} to Generative Adversarial Imitation Learning (GAIL) with state-only demonstrations, later applied to quadrupedal locomotion \cite{vollenweider2022advanced}. \cite{luo2024smpl} highlights the need for high-quality morphologically similar demonstrations and susceptibility of \cite{peng2021amp} to local optima with increased task complexity. Furthermore, with a fixed set of demonstrations, the policy is restricted of pre-generated references, limiting RL's exploration and hindering emergent behaviors crucial for real-robot control, as demonstrated by from-scratch RL methods \cite{siekmann2021blind, cheng2023extreme,hoeller2024anymal}. Thus, applying existing reference-guided methods to morphologically unique robots (like Hector) remains challenging. Hence, we propose a reference-guided policy optimization using closed-loop state-reference generators(oracles) that can be queried dynamically to produce references of arbitrary quality from any state, with a novel hyperparameter to address local optima in complex tasks.

\textbf{Multi-mode Control}: Classical multi-mode control \cite{koo2001multi,asarin2000effective}involves switching among a finite set of pre-designed controllers to address high-level tasks, creating a pseudo-hybrid system. In legged robot control, this combinatorial decision-making manifests as selecting an optimal contact sequence. For locomotion with a preplanned schedule, mature model-based methods exist for trajectory optimization \cite{ponton2021efficient,meduri2023biconmp} and tracking control \cite{grandia2023perceptive}. Model-free methods often leave control multi-modeity to emerge implicitly \cite{rudin2022advanced, cheng2023extreme}, lacking a methodical synthesis. \cite{hoeller2024anymal} trains multiple low-level controllers and a high-level mode-switching policy for quadrupedal parkour, requiring diverse reward shaping and training routines.\cite{krishna2023learning} shows that a ``fixed" set of controllers limits emergent modes and complex transition maneuvers, introducing a single multi-mode policy for finite modes and transitions to handle new tasks zero-shot. We extend this by proposing a reference-generating hybrid automaton (oracles) to achieve a single policy that learns modes with ``infinite" parameter variations and transitions through reference-guided policy optimization. Unlike switching fixed controllers, we hypothesize that reference-guided exploration can better accommodate emergent control modes.


% Unlike a fixed set of controllers, we hypothesize that reference-guided exploration can accommodate emergent modes in a policy. 
% Compared to committing to a fixed set of controllers, we hypothesise that reference-guided GPO should leave room for emergent modes while still being regularized. 
% We extend \cite{krishna2023learning} and are interested in synthesizing a single policy that could learn a finite set of control modes with their "infinite" parameter variations and the corresponding transitions. Thus, for a given task, we propose designing an oracle as a hybrid automaton, generating continuous references for each mode variant and discrete transitions between modes to later perform reference-guided policy optimization.  

% \textbf{multi-mode Control}: Classical multi-mode control \cite{koo2001multi,asarin2000effective} involves switching among a finite set of pre-designed controllers for high-level tasks, creating a pseudo-hybrid system. In legged robots, this manifests as selecting an optimal contact schedule. For locomotion with a preplanned schedule, mature model-based methods exist for trajectory optimization \cite{ponton2021efficient,meduri2023biconmp} and tracking control \cite{grandia2023perceptive}. Model-free contexts often leave control multi-modeity to emerge implicitly \cite{cheng2023extreme}, lacking formal synthesis. \cite{hoeller2024anymal} trains low-level controllers and a high-level mode-switching policy for quadrupedal parkour, requiring diverse reward shaping. \cite{krishna2023learning} shows that fixed controllers limit emergent modes and transitions, introducing a single multi-mode policy for finite modes and transitions to handle new tasks zero-shot. We extend this by proposing a reference-generating hybrid automaton (oracles) to achieve a unified policy with "infinite" parameter variations and transitions through reference-guided policy optimization. Unlike fixed controllers, we hypothesize that reference-guided exploration better accommodates emergent modes.
